Representation Learning in Deep RL via Discrete Information Bottleneck

Several self-supervised representation learning methods have been proposed for reinforcement learning (RL) with rich observations. For real-world applications of RL, recovering underlying latent states is crucial, particularly when sensory inputs contain irrelevant and exogenous information. In this work, we study how information bottlenecks can be used to construct latent states efficiently in the presence of task-irrelevant information. We propose architectures that utilize variational and discrete information bottlenecks, coined as RepDIB, to learn structured factorized representations. Exploiting the expressiveness bought by factorized representations, we introduce a simple, yet effective, bottleneck that can be integrated with any existing self-supervised objective for RL. We demonstrate this across several online and offline RL benchmarks, along with a real robot arm task, where we find that compressed representations with RepDIB can lead to strong performance improvements, as the learned bottlenecks help predict only the relevant state while ignoring irrelevant information.

==> app_algo.tex <==


\section{Algorithm}
\label{sec:app_algo}
$\modelname$ can be integrated on any existing self supervised learning objectives for representations, to reap benefits of the compositional structure for either exploration during pre-training, or for downstream tasks. In this work, we mostly show benefits of $\modelname$ integrated on top of the Proto-RL algorithm \cite{yarats2021protorl}. Algorithm \ref{algo:algo} shows (changes in blue) the additional steps required to integrate the variational information bottleneck (VIB) and discretization bottleneck on the Proto-RL baseline. Furthermore, for structured exploration by using the learnt latent representations, algorithm \ref{algo:algo_intrin_reward} shows how the intrinsic reward based on entropy maximization can be modified to have additional structure, on top of the exploration objective used in Proto-RL.


\begin{algorithm}[t]
    \caption{ProtoRL with Vector Quantization and Variational Information Bottleneck}
   \label{algo:algo}
\begin{algorithmic}[1]
  \STATE Initialize replay buffer $D_\text{explore}$, $D_\text{task}$
  \STATE Initialize critic network $Q_\phi$, explore actor network $\pi_{\theta}$, encoder $f_{\xi}$, and predictor $f_{p}$
  \STATE (Stage I: Pretraining VQ and VIB modules)
  \textcolor{blue}{
  \FOR {k = 1, 2, ..., m}
  \STATE Rollout with policy $\pi_{\theta}$
  \STATE Collect experience in $D_\text{explore}$ using $\pi_\theta$ in the environment
%   \STATE Use an intrinsic reward bonus for exploration - ProtoRL vs Ours with discrete embeddings
  \STATE Sample batch $(s, s') \sim D_\text{explore}$
  \STATE Output representations $z_{s}=f_p(f_{\xi}(s))$ and $z_{s'}=f_p(f_{\xi}(s'))$
  \IF {use Variational Information Bottleneck}
%   \STATE Output reparameterized representation $\hat{z}_{s}$ and $\hat{z}_{s'}$  \textcolor{red}{using Variational Information Bottleneck (VIB)}:
    \STATE Divide state representation $z_s$ into two parts: $\mu_s$ and $\sigma_s$
    \STATE Use reparameterization trick to get variational approximation:
    \begin{equation}
        \hat{z}_{s}=\mu_s + \sigma_s \epsilon, \epsilon\sim \mathcal{N}(0,1)
    \end{equation}
    \STATE Output embedding $\hat{z}_{s}=f(\hat{z}_{s})$ with a linear layer $f$, do the same for representation $z_{s'}$ and output embedding $\hat{z}_{s'}$
  \STATE Compute VIB loss $\mathcal{L}_{\mathrm{gaussian}}=D_\text{KL}(p(\hat{z}|z)||q(\hat{z}|z))$, where we set $q(\hat{z}|z)$ as unit Gaussian.
  \ENDIF
  \STATE Output discrete state embedding $\tilde{z}_s$ and $\tilde{z}_{s'}$ using Discretization Bottleneck
  \STATE Compute the loss function and update the corresponding modules:
  \begin{equation}
      \mathcal{L}=\mathcal{L}_{\mathrm{discretization}} + \mathcal{L}_{\mathrm{gaussian}}
  \end{equation}
  \ENDFOR}
  \STATE (Stage II: Pretraining encoder modules)
  \FOR {k = m, m+1, ..., n}
  \STATE Collect experience in $D_\text{explore}$ using $\pi_\theta$ in the environment
  \STATE Sample batch $(s_t, a_t, r_t, s_{t+1}) \sim D_\text{explore}$
 \textcolor{blue}{ \IF {use Variational Information Bottleneck}
  \STATE Do the same as in Stage I, output embedding $\hat{z}_{s}$ and $\hat{z}_{s'}$
  \ENDIF}
  \STATE Output discrete state embedding $\tilde{z}_s$ and $\tilde{z}_{s'}$ using (Discretization Bottleneck)
  \STATE Compute ProtoRL loss $\mathcal{L}_{\mathrm{proto}}=-q_{s'}\log p_{s}$, where $q_{s'}$ is a target probability vector using prototypes, $p_{s}$ is a probability vector over prototypes
  \STATE Update representation with total loss: $\mathcal{L} = \mathcal{L}_{\mathrm{proto}}\textcolor{blue}{ + \mathcal{L}_{\mathrm{discretization}} + \mathcal{L}_{\mathrm{gaussian}}}$
  \STATE Compute intrinsic reward $r_\text{int}$ with Algorithm~\ref{algo:algo_intrin_reward}
  \STATE Update $Q_{\phi}$ and $\pi_{\theta}$ with intrinsic reward $r_\text{int}$ only
  
  \ENDFOR
  \STATE (Stage III: Finetuning on downstream tasks)
  \FOR {k = n, n+1, ..., K}
  \STATE Collect experience in $D_\test{task}$ using $\pi_\theta$ in the environment
  \STATE Sample batch $(s, a, r, s') \sim D_\text{task}$
   \textcolor{blue}{ \IF {use Variational Information Bottleneck}
  \STATE Output embedding $\hat{z}_{s}$ and $\hat{z}_{s'}$
  \ENDIF}
  \STATE \textcolor{blue}{Output discrete state embedding $\tilde{z}_s$ and $\tilde{z}_{s'}$ using fixed pre-trained discretization bottleneck}
  \STATE Update $Q_{\phi}$ and $\pi_{\theta}$ with external environment reward $r$ using any RL algorithm 
  \ENDFOR
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
    \caption{Compute Intrinsic reward with Vector Quantization and Variational Information Bottleneck}
  \label{algo:algo_intrin_reward}
    \begin{algorithmic}[1]
    \STATE Input: current state representation $z_s$
    \textcolor{blue}{\IF {use Variational Information Bottleneck}
    \STATE Divide state representation $z_s$ into two parts: $\mu_s$ and $\sigma_s$
    \STATE Output deterministic embedding $\hat{z}_{s}=\mu_s$ and pass it to a parameterized linear layer $f_l$:   $\hat{z}_{s}=f_l(\hat{z}_{s})$ 
  \ENDIF
  \STATE Output discrete state embedding $\tilde{z}_s$ using  Discretization Bottleneck}
  \STATE Compute Nearest Neighbor (NN) based entropy estimator as intrinsic reward:
  \begin{equation}
      \hat{r}=\left\|\tilde{z}_{s}-\mathrm{NN}_{k, \boldsymbol{Q}}\left(\tilde{z}_{s}\right)\right\|
  \end{equation}
  \STATE Output: intrinsic reward $\hat{r}$ 
\end{algorithmic}
\end{algorithm}




\clearpage
\section{Pseudocode and Implementation}

(a) code snippet of gaussian bottleneck:
\lstinputlisting[language=Python]{codes/gb.py}

(b) code snippet of computing intrinsic reward:
\lstinputlisting[language=Python]{codes/compute_int_r.py}

(c) code snippet of update proto:
\lstinputlisting[language=Python]{codes/update_proto.py}


